Metric Geometry of Finite Subset Spaces

If $X$ is a (topological) space, the $n$th finite subset space of $X$, denoted by $X(n)$, consists of $n$-point subsets of $X$ (i.e., nonempty subsets of cardinality at most $n$) with the quotient topology induced by the unordering map $q:X^n\to X(n)$, $(x_1,\cdots,x_n)\mapsto\{x_1,\cdots,x_n\}$. That is, a set $A\subset X(n)$ is open if and only if its preimage $q^{-1}(A)$ is open in the product space $X^n$. Given a space $X$, let $H(X)$ denote all homeomorphisms of $X$. For any class of homeomorphisms $C\subset H(X)$, the $C$-geometry of $X$ refers to the description of $X$ up to homeomorphisms in $C$. Therefore, the topology of $X$ is the $H(X)$-geometry of $X$. By a ($C$-) geometric property of $X$ we will mean a property of $X$ that is preserved by homeomorphisms of $X$ (in $C$). Metric geometry of a space $X$ refers to the study of geometry of $X$ in terms of notions of metrics (e.g., distance, or length of a path, between points) on $X$. In such a study, we call a space $X$ metrizable if $X$ is homeomorphic to a metric space. Naturally, $X(n)$ always inherits some aspect of every geometric property of $X$ or $X^n$. Thus, the geometry of $X(n)$ is in general richer than that of $X$ or $X^n$. For example, it is known that if $X$ is an orientable manifold, then (unlike $X^n$) $X(n)$ for $n>1$ can be an orientable manifold, a non-orientable manifold, or a non-manifold. In studying geometry of $X(n)$, a central research question is "If $X$ has geometric property $P$, does it follow that $X(n)$ also has property $P$?". A related question is "If $X$ and $Y$ have a geometric relation $R$, does it follow that $X(n)$ and $Y(n)$ also have the relation $R$?". (Truncated)

==> chaptersTh/append/LoCoWkTp.tex <==
%%################################################################################################################
\section{Geometry of locally convex spaces: Weak topologies (\textcolor{red}{Pending})}\label{LoCoWkTp}
%%################################################################################################################
%%################################################################################################################


==> chaptersTh/front/Approval.tex <==
\thispagestyle{empty}
\begin{center}
  Committee Approval Page
\end{center}

%%#######################################################################################
\newpage

==> chaptersTh/front/FrontAlt.tex <==
%%################################################################################################################
\makeatletter
\patchcmd{\@maketitle}{\newpage}{}{}{}  %% Prevents automatic blank page after tiltle page
\makeatother
%%################################################################################################################
\title{Metric Geometry of Finite Subset Spaces}
\author{\large Thesis  submitted to \\[5pt]
\emph{Syracuse University}\\[2cm]
 in partial fulfilment for the award of the degree
 of \\[2cm]
\textsc{\Large{Doctor of Philosophy}} \\[5pt]
  in Mathematics \vspace{0.4cm} \\[1in]
 By\\[5pt] {\Large \sc Earnest Akofor} \\[1em]

Ph.D. Engineering, Syracuse University, 2016\\
Ph.D. Physics, Syracuse University, 2010\\
B.Sc. Physics, University of Buea, 2001\\

\vfill
 \textcolor{red}{December 2019}\\
%%################################################################################################################
%\let\thefootnote\relax\footnotetext{This work has significant contributions due $\cdots$ .}
%%################################################################################################################
}

\date{}

\maketitle
%%################################################################################################################ 

==> chaptersTh/front/FrontGen.tex <==
%%################################################################################################################
\makeatletter
\patchcmd{\@maketitle}{\newpage}{}{}{}  %% Prevents automatic blank page after tiltle page
\makeatother
%%################################################################################################################
\title{Metric Geometry of Finite Subset Spaces}
\author{\large ~\\[1em]
Earnest Akofor\\[2em]
Department of Mathematics\\
Syracuse University, Syracuse, NY 13244, USA \\[1em]
Email: eakofor@syr.edu\\[8em]
(PhD Dissertation)\\ [2em]
\today\\}
%%################################################################################################################

%\begin{abstract} 
%gdgdshjsfjh 
%\end{abstract}
%\subjclass[2010]{hsdhshsjd, hdhdhdh, ...}
%\keywords{Topological space, Subset space, Metric geometry, Lipschitz connectedness, Lipschitz retraction}
%%################################################################################################################
\maketitle
%%################################################################################################################
%\let\thefootnote\relax\footnotetext{This work has significant contributions due $\cdots$ .}
%%################################################################################################################ 

==> chaptersTh/front/FrontPublic.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is a sample header for a sample dissertation. Fill in the name,
% and the other information. LaTeX will work out the table of
% content, the list of figures and of tables for you.
%
%\begin{flushright}
%draft 5.0\\
%\today
%\end{flushright}

\thispagestyle{empty}
\begin{center}
{\Large Metric Geometry of Finite Subset Spaces}\\[3em]
{Earnest Akofor}\\[1em]

Department of Mathematics\\
Syracuse University, Syracuse, NY 13244, USA \\
Email: eakofor@syr.edu\\[8em]

(PhD Dissertation)\\
\end{center}
%%################################################################################################################
%\let\thefootnote\relax\footnotetext{This work has significant contributions due $\cdots$ .}
%%################################################################################################################
\newpage
%%################################################################################################################


==> chaptersTh/front/TitlePage_prev.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is a sample header for a sample dissertation. Fill in the name,
% and the other information. LaTeX will work out the table of
% content, the list of figures and of tables for you.
%
%\begin{flushright}
%draft 5.0\\
%\today
%\end{flushright}

\thispagestyle{empty}
\begin{center}
{\Large Metric Goemetry of Finite Subset Spaces}\\[3em]
by\\[2em]
{Earnest Akofor}\\[3em]

Ph.D. Electrical $\&$ Computer Engineering, Syracuse University, 2016\\
Ph.D. Physics, Syracuse University, 2010\\
B.Sc. Physics, University of Buea, 2001\\[4em]

Dissertation\\
Submitted in partial fulfillment of the requirements for the degree of\\
Doctor of Philosophy in Mathematics.\\[4em]
\end{center}

\begin{center}
{Syracuse University}\\
{\textcolor{red}{May ... 2020}}\\[5em]
\end{center}

\begin{flushright}
\parbox{3in}{
\begin{flushright}
Approved \hrulefill\\
% Approved \dotfill\\
Prof. Leonid Kovalev\\[1.5em]
\end{flushright}
Date \hrulefill\\
%Date \dotfill\\
}
\end{flushright}

%%#######################################################################################
\newpage 

==> chaptersTh/front/head.tex <==

%%#######################################################################################
\thispagestyle{empty}
  \begin{center}
    {\large Abstract}\\[1em]
  \end{center}
\begin{quote}
In distributed detection, there does not exist an automatic way of generating optimal decision strategies for non-affine decision functions. Consequently, in a detection problem based on a non-affine decision function, establishing optimality of a given decision strategy, such as a generalized likelihood ratio test, is often difficult or even impossible.

In this thesis we develop a novel detection network optimization technique that can be used to determine necessary and sufficient conditions for optimality in distributed detection for which the underlying objective function is monotonic and convex in probabilistic decision strategies. Our developed approach leverages on basic concepts of optimization and statistical inference which are provided in appendices in sufficient detail. These basic concepts are combined to form the basis of an optimal inference technique for signal detection.

We prove a central theorem that characterizes optimality in a variety of distributed detection architectures. We discuss three applications of this result in distributed signal detection. These applications include interactive distributed detection, optimal tandem fusion architecture, and distributed detection by acyclic graph networks. In the conclusion we indicate several future research directions, which include possible generalizations of our optimization method and new research problems arising from each of the three applications considered.
\end{quote}

\let\thefootnote\relax\footnotetext{\textbf{Keywords}: Function optimization, Statistical inference, Optimal hypothesis testing, Distributed detection}

\begin{comment}
\begin{quote}
In distributed detection, there does not exist an automatic way of generating optimal decision strategies for non-affine decision functions. Consequently, in a detection problem based on a non-affine decision function, establishing optimality of a given decision strategy, such as a generalized likelihood ratio test, can be time consuming.

In this thesis we develop a novel detection network optimization technique that can be used to determine necessary and sufficient conditions for optimality in any distributed detection problem for which the underlying objective function is monotonic and convex in decision probabilities. In order to make the thesis self contained, as well as accessible, we provide appendices containing essential basic concepts of optimization and statistical inference in sufficient detail. In our analysis, these basic concepts are combined to form the basis of an optimal inference technique for signal detection.

We prove a central theorem that characterizes optimality in a variety of distributed detection architectures. We discuss three applications of this result in distributed signal detection. These applications include interactive distributed detection, optimal tandem fusion architecture, and distributed detection by acyclic graph networks. In the conclusion we indicate several future research projects, which include possible generalizations of our optimization method and new research problems arising from each of the three applications considered.
\end{quote}
\end{comment}

\newpage
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% This is a sample header for a sample dissertation. Fill in the name,
% and the other information. LaTeX will work out the table of
% content, the list of figures and of tables for you.
%
%\begin{flushright}
%draft 5.0\\
%\today
%\end{flushright}

\thispagestyle{empty}
\begin{center}
{\Large Optimal Inference for Distributed Detection}\\[3em]
by\\[2em]
{Earnest Akofor}\\[3em]

Ph.D. Physics, Syracuse University, 2010\\
B.Sc. Physics, University of Buea, 2001\\[4em]

Dissertation\\
Submitted in partial fulfillment of the requirements for the degree of\\
Doctor of Philosophy in Electrical $\&$ Computer Engineering.\\[4em]
\end{center}

\begin{center}
{Syracuse University}\\
{July 2016}\\[5em]
\end{center}

\begin{flushright}
\parbox{3in}{
\begin{flushright}
Approved \hrulefill\\
% Approved \dotfill\\
Prof. Biao Chen\\[1.5em]
\end{flushright}
Date \hrulefill\\
%Date \dotfill\\
}
\end{flushright}
\newpage

\thispagestyle{empty}
\begin{center}
  \vspace*{3in}
  \copyright \hspace{5mm} Copyright 2016 Earnest Akofor\\[1.5em]
  All rights reserved
\end{center}

%%#######################################################################################
\newpage
\thispagestyle{empty}
\begin{center}
  Committee Approval Page
\end{center}

\newpage
%%#######################################################################################
%\thispagestyle{empty}
\vskip 2cm
\begin{center}
\textbf{Acknowledgments}
\end{center}
\begin{quote}
    The author would like to acknowledge the generous support from the National Science Foundation under Grant CCF1218289, the Army Research Office under Grant W911NF-12-1-0383, and the Air Force Office of Scientific Research, Arlington, VA, USA, under Grant FA9550-10-1-0458.
\end{quote}

\newpage
%%#######################################################################################
\tableofcontents
\listoffigures
%\listoftables

